Engineering optically active defects in hexagonal boron nitride using focused ion beam and water

Hexagonal boron nitride (hBN) has emerged as a promising material platform for nanophotonics and quantum sensing, hosting optically-active defects with exceptional properties such as high brightness and large spectral tuning. However, precise control over deterministic spatial positioning of emitters in hBN remained elusive for a long time, limiting their proper correlative characterization and applications in hybrid devices. Recently, focused ion beam (FIB) systems proved to be useful to engineer several types of spatially-defined emitters with various structural and photophysical properties. Here we systematically explore the physical processes leading to the creation of optically-active defects in hBN using FIB, and find that beam-substrate interaction plays a key role in the formation of defects. These findings are confirmed using transmission electron microscopy that reveals local mechanical deterioration of the hBN layers and local amorphization of ion beam irradiated hBN. Additionally, we show that upon exposure to water, amorphized hBN undergoes a structural and optical transition between two defect types with distinctive emission properties. Moreover, using super-resolution optical microscopy combined with atomic force microscopy, we pinpoint the exact location of emitters within the defect sites, confirming the role of defected edges as primary sources of fluorescent emission. This lays the foundation for FIB-assisted engineering of optically-active defects in hBN with high spatial and spectral control for applications ranging from integrated photonics, to quantum sensing to nanofluidics.

==> FIB hBN paper v1/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
